PaddleSpeech: An Easy-to-Use All-in-One Speech Toolkit

PaddleSpeech is an open-source all-in-one speech toolkit. It aims at facilitating the development and research of speech processing technologies by providing an easy-to-use command-line interface and a simple code structure. This paper describes the design philosophy and core architecture of PaddleSpeech to support several essential speech-to-text and text-to-speech tasks. PaddleSpeech achieves competitive or state-of-the-art performance on various speech datasets and implements the most popular methods. It also provides recipes and pretrained models to quickly reproduce the experimental results in this paper. PaddleSpeech is publicly avaiable at https://github.com/PaddlePaddle/PaddleSpeech.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty *.cls)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
#	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
#	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	#pdflatex si
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "5 5 5 5" main.pdf
	# open main-crop.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

paper.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=1 -dLastPage=12 main.pdf

si.pdf:	${target}.pdf
	gs -q -sPAPERSIZE=letter -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ -dFirstPage=13 -dLastPage=20 main.pdf




==> archive/experiments.tex <==
%%

\section{Experiments}

In this section, we compare the performance of all models in PaddleSpeech with other popular implementations in five speech-related tasks, including sound classification, speech recognition, punctuation, speech translation, and speech synthesizing.
All experiments in this sections include details on data preparation, evaluation metrics, and implementation to enhance the reproducibility.%
\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples}}

% \blue{(Chen, XiaoJie)}
\subsection{Sound Classification}
Sound Classification is a task to recognize particular sounds, including recognizing speech commands \cite{Warden2018SpeechCA}, environment sounds \cite{Piczak2015ESCDF}, identifying musical instruments \cite{Engel2017NeuralAS}, and finding birdsongs \cite{Stowell2018AutomaticAD}.

% which dataset & how preprocess
\paragraph{Datasets}
In this section, we analyze the performance of PaddleSpeech in Sound Classification on ESC-50 dataset \cite{Piczak2015ESCDF}.
The ESC-50 dataset is a labeled collection of 2000 environmental 5-second audio recordings consisting of 50 sound events, such as "Dog", "Cat", "Breathing" and "Fireworks", with 40 recordings per event.

\paragraph{Data Preprocessing}
First, we resample all audio recordings to 32 kHz, and convert them to monophonic to be consistent with the PANNs trained on AudioSet \cite{Kong2020PANNsLP}. 
And then we transform the recordings into log mel spectrograms: STFT is applied on the waveforms with a Hamming window of size 1024 and a hop size of 320 samples.
This configuration leads to 100 frames per second. Following \cite{Kong2019CrosstaskLF}, we apply 64 mel filter banks to calculate the log mel spectrogram.

% details of modeling, training, inference
\paragraph{Implementation}
PANNs \cite{Kong2020PANNsLP} are one of the pre-trained CNN models for audio-related tasks, which is characterized in terms of being trained with the AudioSet \cite{Gemmeke2017AudioSA}.
PANNs are useful for the tasks where only a limited number of training clips are provided.
In this case, We fine-tune all parameters of a PANN for the environment sounds classification task.
All parameters are initialized from the PANN, except the final fully-connected layer which is randomly initialized.
Specifically, we implement 6-, 10- and 14-layer CNNs \cite{Kong2020PANNsLP}.
\begin{itemize}
    \item CNN6:
    consists of 4 convolutional layers with a kernel size of $5 × 5$.
    \item CNN10:
    consists of 4 convolutional blocks. Each convolutional block consists of 2 convolutional layers with a kernel size of $3 × 3$.
    \item CNN14:
    consists 6 convolutional blocks. Each convolutional block consists of 2 convolutional layers with a kernel size of $3 × 3$.
\end{itemize}
Each convolutional block consists of 2 convolutional layers with a kernel size of $3 × 3$.
Batch normalization is applied between each convolutional layer, and the ReLU nstreamingarity is used to speed up and stabilize the training.
We apply average pooling of size of 2 × 2 to each convolutional block for downsampling, as $2 × 2$ average pooling has been shown to outperform $2 × 2$ max pooling \cite{Kong2019CrosstaskLF}.
% The batch size of finetuning is 16, and the learning rate is $5 \times 10 ^{-5}$.

% \paragraph{Hyperparameter}
% \begin{itemize}
%     \item ESC-50
%     \begin{itemize}
%         \item cls0\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/esc50/cls0/conf/panns.yaml}}
%     \end{itemize}
% \end{itemize}

% \paragraph{Metrics}

\paragraph{Results}
We report 5-fold cross validation accuracy values on ESC-50 dataset.
As shown in Table \ref{tab:esc50}, PANNs-CNN14 achieves 0.9500 5-fold cross validation accuracy that is comparable to the current state-of-the-art method \cite{Gong2021ASTAS}.

\begin{table}
\small
\begin{center}
\begin{tabular}{ll}
\toprule
Model                       & Accuracy \\
\midrule
AST-P \citep{Gong2021ASTAS} & $95.6 \pm 0.4$ \\
\midrule
PANNs-CNN14                 & 95.00   \\
PANNs-CNN10                 & 89.75   \\
PANNs-CNN6                  & 88.25   \\
\bottomrule
\end{tabular}
\caption{5-fold cross validation accuracy of ESC-50}
\label{tab:esc50}
\end{center}
\end{table}

\begin{table*}[t]
\small
\centering
\begin{tabular}{llcllll}
\toprule
Data & Model & Streaming & Test Data & Language Model & CER & WER \\
\midrule
\multirow{4}{*}{Aishell}
& DeepSpeech2 & Y & test & char 5-gram%\footnote{\url{https://deepspeech.bj.bcebos.com/zh_lm/zh_giga.no_cna_cmn.prune01244.klm}}
& 8.0 & -  \\
& DeepSpeech2 & N & test & char 5-gram%\footnote{\url{https://deepspeech.bj.bcebos.com/zh_lm/zh_giga.no_cna_cmn.prune01244.klm}}
& 6.4 & - \\
& \red{Conformer}%(效果一般，酌情使用)
& N & test & - & 5.6 & -  \\
& Transformer & N & test & - & 5.23 & -\\
\midrule
\multirow{4}{*}{Librispeech}
& DeepSpeech2 & N & test-clean & word 5-gram%\footnote{\url{https://deepspeech.bj.bcebos.com/en_lm/common_crawl_00.prune01111.trie.klm}}
& - & 7.25  \\
& Conformer & N & test-clean & - & - & 3.37  \\
& Transformer & N & test-clean & - & - & 3.81 \\
& Transformer (add pitch) & N & test-clean & TransformerLM%\footnote{\url{https://deepspeech.bj.bcebos.com/transformer_lm/transformerLM.pdparams}}
& - & 2.40 \\
& SpeechBrain & N & test-clean & unk%\footnote{\url{https://deepspeech.bj.bcebos.com/transformer_lm/transformerLM.pdparams}}
& - & 2.46 \\
% \midrule
% \multirow{1}{*}{TIMIT}
% & Transformer & N & test & - & - & - & 18.23 \\
\bottomrule
\end{tabular}
\caption{ WER/CER of Aishell, Librispeech for ASR Task}
\label{tab:asr-result}
\end{table*}

% \blue{(Huang, YuXin)}
\subsection{Automatic Speech Recognition}

Automatic Speech Recognition(ASR) is a task to transcribe the audio content to text in the same language.

\paragraph{Datasets}
We conduct the ASR experiments on three major datasets as follows. 
\begin{itemize}
    \item
        \textbf{librispeech}\footnote{\url{http://www.openslr.org/12/}}
        \citep{panayotov2015librispeech}
        The dataset contains 1000 hours speech data.
        Three are two kinds data in librispeech dataset, which are clean speech and other not clean speech.
        The whole dataset are divided into 3 training sets (100h clean, 360h clean, 500h other), 2 validation sets (clean, other) and 2 test sets (clean, other).
    \item
        \textbf{AISHELL-1}\footnote{\url{http://www.aishelltech.com/kysjcp}}
        \citep{bu2017aishell}
        The dataset contains 178 hours speech data.
        400 speakers from different accent areas in China participate in the recording.
        The dataset is divided into training set (340 speakers), validation set (40 speakers) and test set (20 speakers).
    % \item
    %     \textbf{TIMIT} The original TIMIT corpus contains 3696 and 192
    %     phonetically transcribed utterances for the training and test sets respectively.
    %     We process the phonememes and extract the validation set following kaldi recipe. \footnote{\url{https://github.com/kaldi-asr/kaldi/tree/master/egs/timit}}
    %     \citep{linguistic1990darpa}
    
\end{itemize}

\paragraph{Data Preprocessing}
For English data, the vocabulary dictionary is composed of 26 English characters.
For mandarin, the vocabulary dictionary is composed of Chinese characters statistics from the training set.
Both two kinds of datasets added three additional characters, which are \texttt{<'>}, \texttt{<space>}, \texttt{<blank>} and \texttt{<eos>}.
For cepstral mean and variance normalization (CMVN), a subset of or full of the training set is selected and be used to compute the feature mean and std. 
For feature extraction, three methods are implemented, which are linear (FFT without using filter bank), fbank and mfcc.
Currently, the released deepspeech2 model uses linear, but Transformer and Conformer models use fbank.

\paragraph{Implementation}

We implement both streaming and non-streaming Deepspeech2 \citep{amodei2016deep}.
The non-streaming model has 2 convolution layers and 3 LSTM layers. 
The streaming model has 2 convolution layers and 5 LSTM layers.
The Conformer and Transformer are implemented as \citet{zhang2020unified} with 12 encoder layers and 6 decoder layers.
% The Transformer used on TIMIT dataset has both 6 encoder and decoder layers.
% All these models support streaming and non-streaming recognition.
% For decoding method, Deepspeech2 models use ctc-beam-prefix decoding.
% Conformer and Transformer model use 4 kinds of decoding methods including ctc-greedy-search, ctc-prefix-beam-search, attention, and attention-rescoring.
% \red{(4 dec? which one?)}

% \paragraph{hyperparameter}
% \begin{itemize}
%     \item librispeech
%     \begin{itemize}
%         \item asr0% deepspeech2 Streaming/Non-Streaming
%         \footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/conf}}
%         The model use DeepSpeech2 architecture.
%         For non-streaming model, the model has 2 convolution layers and 3 LSTM layers. 
        
%         % 训练
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/conf/deepspeech2_online.yaml
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/conf/deepspeech2.yaml
%         % 解码
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/conf/tuning/chunk_decode.yaml
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/conf/tuning/decode.yaml
        
%         \item asr1% transformer/conformer Streaming/Non-Streaming %
%         \footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples/librispeech/asr1/conf}}%
%         The model use Conformer and Transformer architecture.
%         For two kinds of models, they use 12 encoder blocks and 6 decoder blocks.
%         \item asr2% transformer/conformer Streaming/Non-Streaming with Kaldi feature
%         \footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples/librispeech/asr2/conf}}
%         The models use Transformer architecture. The difference between the asr2 model is that asr2 model use pitch as additional feature and use additional language model for decoding.
        
%     \end{itemize}
%     \item aishell
%     \begin{itemize}
%         \item asr0\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples/aishell/asr0/conf}}
%         The model use DeepSpeech2 architecture.
%         For non-streaming model, the model has 2 convolution layers and 3 GRU layers.
%         For streaming model, the model has 2 convolution layers and 5 LSTM layers.
%         \item asr1\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples/aishell/asr1/conf}}
%         The model use Conformer and Transformer architecture. For two kinds of models, they use 12 encoder blocks and 6 decoder blocks.
%     \end{itemize}
    
%     \item timit 
%     \begin{itemize}
%     \item asr1\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/tree/develop/examples/timit/asr1/conf}}
%     The models use Transformer architecture. It use 6 encoder blocks and 6 decoder blocks.
%     \end{itemize}
% \end{itemize}

\paragraph{Results}
We report word error rate (WER) and character error rate (CER) for librispeech (English) and Aishell (Mandarin) speech recgonition correspondingly.
% For TIMIT, we report the \red{phoneme error rate} (PER).
As shown in Table \ref{tab:asr-result}, Conformer and Transformer are obviously better than DeepSpeech2.
An experiment on Aishell show that the steaming mode of DeepSpeech2 does hurt performance.
Another experiment on Librispeech show that adding pitch as additional feature significantly decrease the WER.
\red{(NO RELATED WORK)}

\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccccccc}
\toprule
\textbf{Frameworks}                                    & \textbf{De}   & \textbf{Es}   & \textbf{Fr}   & \textbf{It}   & \textbf{Nl}   & \textbf{Pt}   & \textbf{Ro}   & \textbf{Ru}   \\
\midrule
ESPnet-ST \cite{inaguma2020espnet}       & 22.9 & \textbf{28.0} & 32.8 & \textbf{23.8} & \textbf{27.4} & 28.0 & 21.9 & \textbf{15.8} \\
fairseq-ST \cite{wang-etal-2020-fairseq} & 22.7 & 27.2 & 32.9 & 22.7 & 27.3 & 28.1 & 21.9 & 15.3 \\
NeurST \cite{zhao-etal-2021-neurst}      & 22.8 & 27.4 & \textbf{33.3} & 22.9 & 27.2 & 28.7 & \textbf{22.2} & 15.1 \\
\midrule
PaddleSpeech                             & \textbf{23.0} & 27.4 & 32.9 & 22.9 & 26.7 & \textbf{28.8} & \textbf{22.2} & 15.4 \\
\bottomrule
\end{tabular}
\caption{Case-sensitive detokenized BLEU scores on MuST-C \textit{tst-COMMON}.}
\label{tab:mustc}
\end{table*}

% \begin{itemize}
%     \item librispeech
%     \begin{itemize}
%         \item asr0
%         % deepspeech2 Streaming/Non-Streaming 
%         DeepSpeech2 non-streaming model is released.
%         It use word 5-gram language model for ctc-prefix-beam-search.
%         The WER of the released model is 7.25\%. 
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr0/RESULTS.md
        
%         \item asr1
%         % transformer/conformer Streaming/Non-Streaming 
%         Conformer non-streaming and Transformer non-streaming model are released.
%         The Conformer model get 3.37\% WER and the Transformer model get 3.81\% WER.
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr1/RESULTS.md
%         \item asr2
%         % transformer/conformer Streaming/Non-Streaming with Kaldi feature  
%         The Transformer (add pitch) is released.
%         It add pitch as additional feature and use Transformer language model for decoding.
%         The WER of the model is 2.40\%.
%         %https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/librispeech/asr2/RESULTS.md
%     \end{itemize}
%     \item aishell
%     \begin{itemize}
%         \item asr0
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/aishell/asr0/RESULTS.md
%         DeepSpeech2 non-streaming model and DeepSpeech2 streaming model are released.
%         The two models use char 5-gram language model for decoding.
%         The WER of the non-streaming model is 6.4\% CER.
%         The WER of the streaming model is 8.0\% CER.
%         \item asr1
%         % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/aishell/asr1/RESULTS.md
%         Conformer non-streaming and Transformer non-streaming model are released.
%         The Conformer model get 5.6\% CER and the Transformer model get 5.23\% CER.
%     \end{itemize}
%     \item timit
%     % https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/timit/asr1/RESULTS.md}
%     Transformer non-streaming is released. The PER of the model is 18.23\%.
% \end{itemize}

% \blue{(Chen, XiaoJie)}
\subsection{Punctuation Restoration}

Punctuation restoration is a common post-processing problem for ASR systems.
It is important to improve the readability of the transcribed text for the human reader and facilitate NLP tasks.

\paragraph{Datasets}
We conduct experiment on IWSLT2012-zh\footnote{\url{https://hltc.cs.ust.hk/iwslt/}} dataset.
IWSLT2012-zh contains 150,000 Chinese sentences with punctuations.
We select comma, period, and question marks as restore target in this task, so we replace other punctuations with these 3 marks before training a model.
We split all Chinese sentences into into training, evaluating and testing sets with 147,000, 2,000 and 1,000 samples respectively. 


% details of modeling, training, inference
\paragraph{Implementation}
We formulate the problem of punctuation restoration as a sequence labeling task with four target classes including \texttt{EMPTY}, \texttt{COMMA}, \texttt{PERIOD}, and \texttt{QUESTION} \citep{Nagy2021AutomaticPR}.
ERNIE (Enhanced Representation through kNowledge IntEgration) \cite{Sun2019ERNIEER} is a novel language representation model.
Experimental results \cite{Sun2019ERNIEER} show that ERNIE outperforms other baseline methods, achieving new state-of-the-art results on five Chinese natural language processing tasks including natural language inference, semantic similarity, named entity recognition, sentiment analysis and question answering.
We finetune an ERNIE model for this Chinese sequence task.
More specifically, all parameters are initialized from the ERNIE pretrained model, except the final shared fully-connected layer which is randomly initialized.

% \paragraph{Hyperparameter}
% \begin{itemize}
%     \item IWSLT2012-zh
%     \begin{itemize}
%         \item punc0\footnote{\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/iwslt2012/punc0/conf/default.yaml}}
%     \end{itemize}
% \end{itemize}

\paragraph{Results}
We report F1-score values on IWSLT2012-zh dataset.
As shown in Table \ref{tab:iwslt2012-zh-pr}, ERNIE based model achieves 0.6331 overall f1-scores.
In case of each label, it achieves 0.5142, 0.5447 and 0.8406 respectively.
\red{(NO RELATED WORK}
% 用这个做为对比吧，模型结构比我们的大 https://github.com/yuboona/Chinese-Punctuation-Restoration-with-Bert-CNN-RNN#4-experiments-results)。
% 另一篇论文
% Zhang Z, Liu J, Chi L, et al. Word-level BERT-CNN-RNN Model for Chinese Punctuation Restoration[C]//2020 IEEE 6th International Conference on Computer and Communications (ICCC). IEEE, 2020: 1629-1633.

\begin{table}[t]
\small
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{lcccc}
\toprule
model & COMMA  & PERIOD & QUESTION & Overall \\
\midrule
BertCRNN
% https://github.com/yuboona/Chinese-Punctuation-Restoration-with-Bert-CNN-RNN#4-experiments-results
& 0.5580 & 0.7517 &  0.7630  &  0.6909  \\
\midrule
ERNIE & 0.5142 & 0.5447 & 0.8406   & 0.6331  \\
\bottomrule
\end{tabular}
\caption{F1-score values on IWSLT2012-zh dataset.}
\label{tab:iwslt2012-zh-pr}
\end{table}

% \blue{(Junkun)}
\subsection{Speech Translation}

\paragraph{Datasets}
In this section, we analyze the performance of PaddleSpeech in Speech Translation on MuST-C dataset \cite{di2019must} with 8 different language translation pairs, which take the English speech as source input. 

\paragraph{Implementation}
We process the raw audios with Kaldi \cite{povey2011kaldi} 
and extract 80-dimensional log-mel filterbanks stacked with 3-dimensional pitch feature
using a 25ms window size and a 10ms step size.
Text is firstly tokenized with Moses tokenizer\footnote{\url{https://github.com/moses-smt/mosesdecoder}} 
and then processed by SentencePiece \cite{kudo2018sentencepiece} with a joint vocabulary 
size of 8K for each language pairs.
We employ the standard Transformer \citep{vaswani2017attention} as the base architecture for the speech translation experiments.
In detail, 
the Transformer model has 12 encoder layers that follows 2 layers of 2D convolution
with kernel size 3 and stride size 2,
and 6 decoder layers.
Each layer contains 4 attention heads with size of 256.
The parameters of the encoder are initialized from a pretrained ASR model.

\paragraph{Results}
We report detokenized case-sensitive BLEU\footnote{\url{https://github.com/mjpost/sacrebleu}}.
As shown in Table \ref{tab:mustc}, 
PaddleSpeech can achieve competitive results with other frameworks.

% \blue{(Yuantian)}
\subsection{Text-To-Speech}

TTS system mainly includes three modules: Text Frontend, Acoustic model and Vocoder. 
The main processes of TTS include:

1. Convert the original text into characters/phonemes, through the text frontend module.

2. Convert characters/phonemes into acoustic features, such as linear spectrogram, mel spectrogram, LPC features, etc. through Acoustic models.

3. Convert acoustic features into waveforms through Vocoders.

A simple text frontend module can be implemented by rules. Acoustic models and vocoders need to be trained. The models provided by PaddleSpeech TTS are acoustic models and vocoders.

\paragraph{Datasets}

\begin{table*}[t]
\small
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{clccrcr}
\toprule
\textbf{Language} & \textbf{Data} & \textbf{\# Hours}  & \textbf{\# Sentences} & \textbf{Size (GB)} & \textbf{\# Speaker} & \textbf{Sample Rate}   \\
\midrule
\multirow{2}{*}{Mandarin} & CSMSC\footnote{\url{https://www.data-baker.com/open_source.html}} & 12 & 10,000 & 2.14   & 1  & 48,000 Hz  \\
  & AISHELL-3\footnote{\url{http://www.aishelltech.com/aishell_3}} & 85 & 88,035 & 17.75 & 218 & 44,100 Hz \\ \midrule
\multirow{2}{*}{English} & LJSpeech\footnote{\url{https://keithito.com/LJ-Speech-Dataset/}} & 24 & 13,100 & 2.56  & 1 & 22,050 Hz \\
  & VCTK\footnote{\url{https://datashare.ed.ac.uk/handle/10283/3443}} & 44 & 44,583 & 19.94 & 110 & 48,000 Hz \\
\bottomrule
\end{tabular}
\caption{Statistics of TTS Datasets.}
\label{tab:dataset}
\end{table*}


There are many datasets in TTS. In PaddleSpeech, we mainly focus on Mandarin and English speech synthesis, The relevant main datasets are shown in Table~\ref{tab:dataset}.

\if 0
Mandarin:
\begin{itemize}
    \item CSMSC\footnote{\url{https://www.data-baker.com/open_source.html}}
    \begin{itemize}
    \item Duration/h: 12
    \item Number of Sentences: 10,000
    \item Size: 2.14GB
    \item Speaker: 1 female, ages 20 ~30
    \item Sample Rate: 48 kHz、16bit
    \item Mean Words per Clip: 16
    \end{itemize}
    \item AISHELL-3\footnote{\url{http://www.aishelltech.com/aishell_3}} \citep{shi2020aishell}
    \begin{itemize}
    \item Duration/h: 85
    \item Number of Sentences: 88,035
    \item Size: 17.75GB
    \item Speaker: 218
    \item Sample Rate: 44.1 kHz、16bit
    \end{itemize}
\end{itemize}

English:
\begin{itemize}
    \item LJSpeech\footnote{\url{https://keithito.com/LJ-Speech-Dataset/}} \citep{ljspeech17}
    \begin{itemize}
    \item Duration/h: 24
    \item Number of Sentences: 13,100
    \item Size: 2.56GB
    \item Speaker: 1, age 20 ~30
    \item Sample Rate: 22050 Hz、16bit
    \item Mean Words per Clip: 17.23
    \end{itemize}
    \item VCTK\footnote{\url{https://datashare.ed.ac.uk/handle/10283/3443}} \citep{yamagishi2019cstr}
    \begin{itemize} 
    \item Number of Sentences: 44,583
    \item Size: 10.94GB
    \item Speaker: 110
    \item Sample Rate: 48 kHz、16bit
    \item Mean Words per Clip: 17.23
    \end{itemize}
\end{itemize}
\fi 

We will mainly list the experimental results on CSMSC (Biaobei).

\paragraph{Text Frontend} 

We provide a complete Chinese text frontend module in PaddleSpeech TTS.
A text frontend module mainly includes:
    Text Segmentation,
    Text Normalization (TN),
    Word Segmentation (mainly in Chinese),
    Part-of-Speech,
    Prosody,
    G2P (Grapheme-to-Phoneme, include Polyphone and Tone Sandhi, etc.),
    Linguistic Features/Charactors/Phonemes.

% 其中最重要的模块是 文本正则化 模块和 字音转换（TTS 中更常用 G2P 代指） 模块。

\begin{table*}[tb]
\small
\setlength{\tabcolsep}{0pt}
\centering
\resizebox{2.1\columnwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
 & \textbf{Module} & \textbf{Result} \\
\midrule
\multirow{9}{*}{\rotatebox{90}{\textbf{PaddleSpeech}}} & & \textit{jīn ti\=an} &  sh\`i & & & zu\`i dī & w\=en d\`u & sh\`i &   \\
& \textit{Text} & 今天 & 是 & \textcolor{red}{2020/10/29} & ，& 最低& 温度& 是& \textcolor{blue}{-3°C} & 。  \\
&  {\small\it} & today & is  &    & & lowest & temperature &is& \\ \cmidrule{2-11}
 & & & & \textcolor{red}{\textit{ \`er l\'ing \`er l\'ing n\'ian sh\'i y\`ue \`er sh\'i j\v{i}u r\`i}} & & & & & \textcolor{blue}{\textit{l\'ing xi\`a \;\;\; s\=an \; d\`u}} \\
& \textbf{TN} & 今天 &是 &\textcolor{red}{二\;零\;\;二\;\;零 \; 年 \;\; 十 \;月 \;二\;十\;九 \;日} &，&最低&温度&是 &\textcolor{blue}{零下 \;\;\;\; 三 \;\; 度} &。\\
&  & & & \textcolor{red}{2\;\; 0\;\;\; 0\;\;\; 2\;\; year\; 10 {\scriptsize month} \;\; 29 \;\;\;day} & & & & & \textcolor{blue}{\textit{negative three degree}} \\ \cmidrule{2-11}
& \textbf{WS} & 今天 /& 是 /& 二零二零年 / 十月 / 二十九日 &，& /  最低&温度 /& 是 /& 零下 / 三度 &。\\ \cmidrule{2-11}
& \textbf{G2P} & { jin1 tian1} & { shi4} & { er4 ling2 er4 ling2 nian2 shi4 yue4 er4 shi2 jiu3 ri4} &  & { zui4 di1} & { wen1 du4} & { shi4} & { ling2 xia4 san1 du4} & \\ \midrule
\multicolumn{2}{c}{\textbf{ESPnet}} & jin1 tian1 &  shi4 & 2020/10/29 & & zui4 di1 & wen1 du4 & shi4 & -3°C  \\
\bottomrule
\end{tabular}
}
\caption{An example of the Chinese text preprocessing pipeline for mandarin TTS
of PaddleSpeech and ESPnet. \textbf{TN} stands for the text normalization module, \textbf{WS} stands for the word segmentation module,
\textbf{G2P} stands for the grapheme-to-phoneme module.
The text normalization module for mandarin of ESPnet is not able to correctly 
handle dates (2020/10/29) and temperatures (-3°C).
}
\label{tab:preprocess}
\end{table*}

The text front-end system of PaddleSpeech Text-to-Speech consists of two parts:
text normalization \footnote{The detail of text normalization module for mandarin can be found at： \url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/docs/source/tts/zh_text_frontend.md}}
and Grapheme-to-Phoneme (G2P) system.
Our G2P system consists of a \red{polyphone} module, which uses pypinyin and g2pM, 
and a \red{tone sandhi} module which uses rules based on chinese word segmentations.


\paragraph{Data Preprocessing}

%以 FastSpeech2 为例，PaddleSpeech TTS 声学模型的数据预处理流程主要如下所示
PaddleSpeech TTS uses the following modules for data
preprocessing \footnote{See details in \url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/csmsc/tts3/local/preprocess.sh}}:
1. Forced alignment: we use Montreal-Forced-Aligner for the duration of phonemes,
2. Feature extraction: we extract Mel-spectrogram as features (additional pitch 
and energy features for Fastspeech 2)
3. Compute statistics (mean, diviation) of each feature and do normalization. %计算各个特征的统计特征（均值、标准差）并进行 normalize


\paragraph{Acoustic Model}

Acoustic models can be mainly classified into autoregressive and non-autoregressive models.
At each step, the decoding of the autoregressive model relies on previous predictions,
which leads to longer inference time but relatively better quality.
While the non-autoregressive model generates the outputs in parallel,
so the inference speed is faster, 
but the quality of generated result if relatively poor.

% PaddleSpeech 已经实现的主流声学模型如下:
As shown in Table \ref{tab:intro}, PaddleSpeech has implemented the following commonly used autoregressive acoustic models:
 Tacotron2 and  TransformerTTS,
and non-autoregressive acoustic models: SpeedySpeech, FastPitch, FastSpeech2.
%PaddleSpeech TTS 已经实现了 Tacotron2、TransformerTTS 和 SpeedySpeech 和 FastSpeech2
%后续内容中我们主要以 FastSpeech2 为例，PaddleSpeech TTS 实现的 FastSpeech2 与论文不同的地方在于，我们使用的的是 phone 级别的 pitch 和 energy(与 FastPitch 类似)，这样的合成结果可以更加稳定。


\paragraph{Vocoder}

As shown in Table \ref{tab:intro}, PaddleSpeech has implemented
the following vocoders: 
%PaddleSpeech 已经实现的主流声码器如下:
WaveFlow, Parallel WaveGAN, MelGAN, Style MelGAN, 
Multi Band MelGAN and HiFi GAN.
%PaddleSpeech TTS 主要实现了百度的 WaveFlow 和一些主流的 GAN Vocoder，后续内容中我们主要以 Parallel WaveGAN 为例。

% details of modeling, training, inference
\paragraph{Implementation}

The PadddleSpeech TTS implementation of  FastSpeech 2 adopts some improvement from
FastPitch and uses MFA to calculate the forced alignment (the original FastSpeech 2
paper uses Tacotron 2).
%The hyper-parameters of our mode
%声学模型的模型和训练超参与原始论文不一致（原始论文是 FastSpeech2，但是我们是融合了 FastPitch 的改进，原始论文使用 Tacotron2 获得强制对齐结果，我们使用 MFA 获得），因为使用的数据集不同(论文一般是 LJSpeech 数据集，我们虽然也有 LJSpeech 数据集，但主要是在中文数据集 CSMSC 上的实验，采样率是不同的)、文本前端不同等，但是我们的模型和训练超参数（除了文本前端相关的 lexicon 等）与 espnet 保持一致

%PadddleSpeech TTS 声码器的模型和训练超参与原始论文不一致，因为使用的数据集不同(论文一般是 LJSpeech 数据集，我们虽然也有 LJSpeech 数据集，但主要是在中文数据集 CSMSC 上的实验，采样率是不同的)，但是我们的模型和训练超参数）与 espnet 保持一致

%PadddleSpeech TTS 主要在中英文数据集上做实验，如上述 4 个数据集，其中对于 LJSpeech 数据集，其原始音频采样率是 22.05kHz，我们的实验配置也是 22.05kHz，具体请参考 \url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/ljspeech/voc1/conf/default.yaml}


Please note that the speech feature parameters of the acoustic model and the
vocoder of one TTS pipeline should be the same.
%1. 同一个数据集的声学模型和声码器的音频特征相关配置需要保持一致，才能级联起来合成音频
%音频相关特征，如下所示：
The following is a sample of speech related features' parameters: 
fs: 24000,                % Sampling rate.
n\_fft: 2048,              % FFT size (samples).
n\_shift: 300,             % Hop size (samples). 12.5ms
win\_length: 1200,         % Window length (samples). 50ms
                         % If set to null, it will be the same as fft_size.
window: "hann",           % Window function.
n\_mels: 80,               % Number of mel basis.
fmin: 80,                 % Minimum freq in mel basis calculation. (Hz)
fmax: 7600.               % Maximum frequency in mel basis calculation. (Hz)

% 2.对于声码器，上采样的参数 upsample_scales 各个系数的乘积要等于 n_shift(hop_size, hop_length)



\paragraph{Results}

\begin{table}[t!]
% \small
\centering
\resizebox{\columnwidth}{!}{
% \setlength{\tabcolsep}{1.pt}
\begin{tabular}{c|c c|c}
\toprule
    &   \textbf{ Acoustic Model} & \textbf{Vocoder} & \textbf{MOS} $\uparrow$ \\
\midrule
ESPnet & Fastspeech 2 & PWGAN & 2.55 $\pm$ 0.19 \\ \midrule
     & Tacotron 2  & PWGAN & 3.69 $\pm$ 0.11 \\ % 2,317.14 & 5,024 \\
     & Speedyspeech & PWGAN & 3.79 $\pm$ 0.09 \\ %494.34    & 2,640 \\
     & Fastspeech 2 & PWGAN & 4.25 $\pm$ 0.09 \\
PaddleSpeech & Fastspeech 2 & Style MelGAN & 4.32 $\pm$ 0.10 \\
     & Fastspeech 2 & MB MelGAN & 4.43 $\pm$ 0.09 \\
     & Fastspeech 2 & HiFi GAN & 4.72 $\pm$ 0.08 \\
\midrule
\end{tabular}
}
\caption{The MOS evaluation with 95\% confidence intervals 
for TTS models trained using CSMSC dataset. PWGAN stands for
Parallel WaveGan, MB MelGAN stands for Multi-Band MelGAN.
}
\label{tb:tts}
\end{table}

%We use MOS Score\footnote{\url{https://en.wikipedia.org/wiki/Mean_opinion_score}}
%to evaluate TTS on 14 Chinese sentences for audios synthesized by 7 different models. 
We report the mean opinion score (MOS) for naturalness evaluation 
in Table \ref{tb:tts}. We use the crowdMOS toolkit (Ribeiro et al., 2011), where 14 Chinese samples from these 7 different models were presented to 14 workers on Mechanical Turk.
As shown in Table \ref{tb:tts}, 
PaddleSpeech can largely outperform ESPnet on madarin TTS.
The main reason is that our

%\red{描述一下评测的setup，多少人，多少条；MOS的95\%置信度。14条样例放附录里。说明下espnet这么差是因为文本前端。}
% Vocoder的RTF是否也加上去？
% https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/docs/topic/gan_vocoder/gan_vocoder.ipynb


%\red{(More Details of MOS Setup)}
%PadddleSpeech TTS 主要在中英文数据集上做实验，如上述 4 个数据集，其中对于 LJSpeech 数据集，其原始音频采样率是 22.05kHz，我们的实验配置也是 22.05kHz，具体请参考 \url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/ljspeech/tts3/conf/default.yaml}
%对于其他三个数据集，由于其原始音频的采样率均大于 24k， 所以我们采用的采样率是 24k \footnote{ see 
%details in 
%\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/csmsc/tts3/conf/default.yaml}, 
%\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/aishell3/tts3/conf/default.yaml},
%\url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/vctk/tts3/conf/default.yaml}}.



%\paragraph{Data Preprocessing}
%% details of modeling, training, inference
%以 Parallel WaveGAN 为例，PaddleSpeech TTS 声码器的数据预处理流程主要如下所示(具体请参考 \url{https://github.com/PaddlePaddle/PaddleSpeech/blob/develop/examples/csmsc/voc1/local/preprocess.sh}):  

%\begin{itemize}
%    \item 强制对齐（MFA, Montreal-Forced-Aligner）获得音素对应时长，主要用于删除音频前后的静音
%    \item 提取特征， GAN Vocoder 需要提取的特征是 mel 特征（与 声学模型中的 mel 特征一致）
%    \item 计算特征的统计特征（均值、标准差）并进行 normalize
%\end{itemize}




% Compnents: ESPnet, Fairseq, Neur-ST, DELTA

